Ctrl-Shift: How Privacy Sentiment Changed from 2019 to 2021

People's privacy sentiments influence changes in legislation as well as technology design and use. While single-point-in-time investigations of privacy sentiment offer useful insight, study of people's privacy sentiments over time is also necessary to better understand and anticipate evolving privacy attitudes. In this work, we use repeated cross-sectional surveys (n=6,676) to model the sentiments of people in the U.S. toward collection and use of data for government- and health-related purposes from 2019-2021. After the onset of COVID-19, we observe significant decreases in respondent acceptance of government data use and significant increases in acceptance of health-related data uses. While differences in privacy attitudes between sociodemographic groups largely decreased over this time period, following the 2020 U.S. national elections, we observe some of the first evidence that privacy sentiments may change based on the alignment between a user's politics and the political party in power. Our results offer insight into how privacy attitudes may have been impacted by recent events and allow us to identify potential predictors of changes in privacy attitudes during times of geopolitical or national change.

==> abstract.tex <==
People's privacy sentiments influence changes in legislation as well as technology design and use. While single-point-in-time investigations of privacy sentiment offer useful insight, study of people's privacy sentiments over time is also necessary to better understand and anticipate evolving privacy attitudes. In this work, we use repeated cross-sectional surveys (n=6,676) to model the sentiments of people in the U.S. toward collection and use of data for government- and health-related purposes from 2019-2021. After the onset of COVID-19, we observe significant decreases in respondent acceptance of government data use and significant increases in acceptance of health-related data uses. While differences in privacy attitudes between sociodemographic groups largely decreased over this time period, following the 2020 U.S. national elections, we observe some of the first evidence that privacy sentiments may change based on the alignment between a user's politics and the political party in power. Our results offer insight into how privacy attitudes may have been impacted by recent events and allow us to identify potential predictors of changes in privacy attitudes during times of geopolitical or national change.
